Handling Data-Based Concurrency in Context-Aware Service Protocols

Dependency analysis is a technique to identify and determine data dependencies between service protocols. Protocols evolving concurrently in the service composition need to impose an order in their execution if there exist data dependencies. In this work, we describe a model to formalise context-aware service protocols. We also present a composition language to handle dynamically the concurrent execution of protocols. This language addresses data dependency issues among several protocols concurrently executed on the same user device, using mechanisms based on data semantic matching. Our approach aims at assisting the user in establishing priorities between these dependencies, avoiding the occurrence of deadlock situations. Nevertheless, this process is error-prone, since it requires human intervention. Therefore, we also propose verification techniques to automatically detect possible inconsistencies specified by the user while building the data dependency set. Our approach is supported by a prototype tool we have implemented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{M.R. Mousavi and G. Sala{\"u}n (Ed.): International
Workshop \\ on the  Foundations of Coordination Languages and \\ Software Architectures (FOCLASA 2010).\\
EPTCS 30, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.30.5}{10.4204/EPTCS.30.5}}

